Impact of 3D LiDAR Resolution in Graph-based SLAM Approaches: A Comparative Study

Simultaneous Localization and Mapping (SLAM) is a key component of autonomous systems operating in environments that require a consistent map for reliable localization. SLAM has been a widely studied topic for decades with most of the solutions being camera or LiDAR based. Early LiDAR-based approaches primarily relied on 2D data, whereas more recent frameworks use 3D data. In this work, we survey recent 3D LiDAR-based Graph-SLAM methods in urban environments, aiming to compare their strengths, weaknesses, and limitations. Additionally, we evaluate their robustness regarding the LiDAR resolution namely 64 $vs$ 128 channels. Regarding SLAM methods, we evaluate SC-LeGO-LOAM, SC-LIO-SAM, Cartographer, and HDL-Graph on real-world urban environments using the KITTI odometry dataset (a LiDAR with 64-channels only) and a new dataset (AUTONOMOS-LABS). The latter dataset, collected using instrumented vehicles driving in Berlin suburban area, comprises both 64 and 128 LiDARs. The experimental results are reported in terms of quantitative `metrics' and complemented by qualitative maps.

==> sections/abstract.tex <==
Simultaneous Localization and Mapping (SLAM) is a critical component of autonomous systems operating in environments that require a metric map for reliable localization. SLAM has been extensively studied for several decades, with early LiDAR-based approaches predominantly relying on 2D data, while recent advancements utilize 3D data for improved accuracy and robustness.

In this work, we provide a survey of recent 3D LiDAR-based Graph-SLAM methods in urban environments, with the objective of comparing their strengths, weaknesses, and limitations under varying scan resolutions. Specifically, we evaluate SC-LeGO-LOAM, SC-LIO-SAM, Cartographer, and HDL-Graph SLAM in real-world urban scenarios using the KITTI odometry dataset as well as the AUTONOMOS-LABS dataset. The latter comprises 3D LiDAR data captured with 64- and 128-beam sensors in suburban areas of Berlin.


==> sections/material_methods.tex <==
%\section{Materials and Methodolegies}
\section{Evaluation performance measures}
\label{sec:Materials}

%The predominant metrics employed for the assessment of SLAM or drift within robotic systems encompass Absolute Trajectory Error (ATE) and Relative Trajectory Error (RTE).
The predominant metrics employed for the assessment of SLAM are the Absolute Trajectory Error (ATE) and Relative Trajectory Error (RTE). ATE quantifies the differences between the estimated trajectory and ground-truth poses. ATE can be calculated considering: root-mean-square error (\textit{RMSE}), mean, and median. The key assumptions to calculate the performance measures are: the sequence for the estimated poses of the trajectory is given by $p_i$ while the ground truth trajectory is $g_i$, where each pose represents a position $n$ in the world coordinate system, assuming that both trajectories are aligned and the rotation matrix R is the identity matrix. RTE measures the local accuracy of SLAM over a fixed time interval $\delta$. Thus, considering $P \in SE_3$ as the estimated matrix and $G\in SE_3$ as the ground truth matrix, the relative pose error $R_i$ at timestamp $i$ is:


 For a sequence of $n$ poses, we obtain $m = n - \delta$ relative pose errors, the $\delta$ parameter was set to 10 to calculate for all frames. The RTE is usually divided in two components: rotation and translation. Just like in ATE it calculates the RMSE and mean error, for demonstration we will just show how to calculate RMSE:


To evaluate the processing time in \textit{ms} of each algorithm, we calculated the average time of the main threads and took the highest value, since they are processed in parallel. 

%..On the other hand, the RTE measures$
